Chameleon: a Heterogeneous and Disaggregated Accelerator System for Retrieval-Augmented Language Models

A Retrieval-Augmented Language Model (RALM) combines a large language model (LLM) with a vector database to retrieve context-specific knowledge during text generation. This strategy facilitates impressive generation quality even with smaller models, thus reducing computational demands by orders of magnitude. To serve RALMs efficiently and flexibly, we propose Chameleon, a heterogeneous accelerator system integrating both LLM and vector search accelerators in a disaggregated architecture. The heterogeneity ensures efficient serving for both inference and retrieval, while the disaggregation allows independent scaling of LLM and vector search accelerators to fulfill diverse RALM requirements. Our Chameleon prototype implements vector search accelerators on FPGAs and assigns LLM inference to GPUs, with CPUs as cluster coordinators. Evaluated on various RALMs, Chameleon exhibits up to 2.16$\times$ reduction in latency and 3.18x speedup in throughput compared to the hybrid CPU-GPU architecture. The promising results pave the way for adopting heterogeneous accelerators for not only LLM inference but also vector search in future RALM systems.

==> conclusion.tex <==
\section{Conclusion}


% Retrieval-augmented language models offer compelling advantages but also present unique system design challenges. 
% To address these problems, 
We present Chameleon, an efficient RALM inference engine that integrates two proposed system design principles: accelerator heterogeneity and accelerator disaggregation. Our Chameleon prototype achieves up to 3.18$\times$ speedup in throughput compared to the state-of-the-art systems, paving the way for the adoption of these design principles in future-generation RALM systems.


% Retrieval-augmented language models offer compelling advantages but also present unique system design challenges. To address these problems, we introduce Chameleon, an efficient RALM inference engine that leverages (a) accelerator heterogeneity for high-performance LLM inference and vector retrieval and (b) accelerator disaggregation for system flexibility and resource efficiency. Our Chameleon prototype achieves up to 3.18$\times$ speedup in throughput compared to the state-of-the-art systems. These promising results validate the effectiveness of the proposed design principles and paves the way for the adoption of accelerator heterogeneity and disaggregation in future-generation RALM systems.




%Our Chameleon prototype, implemented on a heterogeneous cluster of CPUs, GPUs, and FPGAs achieves up to 3.18$\times$ speedup in throughput compared to existing state-of-the-art systems. These promising results validate the effectiveness of the proposed design principles, specifically the integration of accelerator heterogeneity and disaggregation, paving the way for the adoption of these principles in future-generation RALM systems.


% Leveraging accelerator heterogeneity and disaggregation, Chameleon enhances RALM inference efficiency for two primary reasons: firstly, it enables efficient execution of both LM inference and retrieval, and secondly, it allows each system component to be scaled independently, satisfying various system requirements of different RALM configurations.


